A MIP Backend for the IDP System

The IDP knowledge base system currently uses MiniSAT(ID) as its backend Constraint Programming (CP) solver. A few similar systems have used a Mixed Integer Programming (MIP) solver as backend. However, so far little is known about when the MIP solver is preferable. This paper explores this question. It describes the use of CPLEX as a backend for IDP and reports on experiments comparing both backends.

==> idp-latex/idp-latex.tex <==
%IMPORTANT: ONLY INCLUDE AS \input{idp-latex/idp-latex}
\usepackage{import}

\subimport{idp-latex/}{includes-no-theorems}
\subimport{idp-latex/}{common-citations}
\subimport{idp-latex/}{theorems}


==> idp-latex/theorems.tex <==
\usepackage{amsthm}

\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{theorem}[thm]{Theorem}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem*{lem*}{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{conjecture}[thm]{Conjecture}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{lemma}[thm]{Lemma}

\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{definition}[thm]{Definition}

\newtheorem{nota}[thm]{Notation}
\newtheorem*{nota*}{Notation}


\newtheoremstyle{example_basic} 
{\topsep} %ABOVESPACE
{\topsep} %BELOWSPACE 
{\normalfont}% Body font 
{0pt}% Indent amount (empty = no indent, \parindent = para indent) 
{\bfseries}% Thm head font 
{.}% Punctuation after thm head 
{5pt plus 1pt minus 1pt}% Space after thm head (\newline = linebreak) 
{}% Thm head spec

\newtheoremstyle{example_contd}
{\topsep} %ABOVESPACE
{\topsep} %BELOWSPACE 
{\normalfont}% Body font 
{0pt}% Indent amount (empty = no indent, \parindent = para indent) 
{\bfseries}% Thm head font 
{.}% Punctuation after thm head 
{5pt plus 1pt minus 1pt}% Space after thm head (\newline = linebreak) 
{\thmname{#1} \thmnumber{ #2}\thmnote{#3} (continued)}% Thm head spec 

\theoremstyle{example_basic} 
\newtheorem{ex}[thm]{Example}
\newtheorem{example}[thm]{Example}
\newtheorem{remark}[thm]{Remark}

\newtheorem{ex*}{Example}
\theoremstyle{example_contd} 
\newtheorem*{ex_continued}{Example}

\theoremstyle{plain}



